BCL: A Cross-Platform Distributed Container Library

One-sided communication is a useful paradigm for irregular parallel applications, but most one-sided programming environments, including MPI's one-sided interface and PGAS programming languages, lack application level libraries to support these applications. We present the Berkeley Container Library, a set of generic, cross-platform, high-performance data structures for irregular applications, including queues, hash tables, Bloom filters and more. BCL is written in C++ using an internal DSL called the BCL Core that provides one-sided communication primitives such as remote get and remote put operations. The BCL Core has backends for MPI, OpenSHMEM, GASNet-EX, and UPC++, allowing BCL data structures to be used natively in programs written using any of these programming environments. Along with our internal DSL, we present the BCL ObjectContainer abstraction, which allows BCL data structures to transparently serialize complex data types while maintaining efficiency for primitive types. We also introduce the set of BCL data structures and evaluate their performance across a number of high-performance computing systems, demonstrating that BCL programs are competitive with hand-optimized code, even while hiding many of the underlying details of message aggregation, serialization, and synchronization.

==> artifact-description.tex <==
\appendices
\section{Artifact Description: PCL: A Distributed Container Library for HPC}

\subsection{Abstract}
This artifact describes all benchmarks of the \bclfullname{} presented in the
SC 2018 paper titled PCL: A Distributed Container Library for HPC.

\subsection{Description}
\subsubsection{Check-list (artifact meta information)}
\begin{itemize}
  \item \textbf{Program} C, C++, Chapel, and UPC, using MPI, SHMEM, and GASNet.
  \item \textbf{Compilation} Compilation with GCC 7.2.0, Chapel 1.16.0,
  Berkeley UPC 2.26.0, Cray MPICH 7.7.0, Cray SHMEM 7.7.0, and GASNet 1.30.0.
  \item \textbf{Datasets} NERSC Meraculous benchmark genomics datasets.
  \item \textbf{Runtime Environment} SUSE Linux Enterprise Server 12 on NERSC Cori
  and Edison.
  \item \textbf{Hardware}
  \begin{itemize}
    \item NERSC's Cori Phase I supercomputer, a Cray XC40.  Each node is equipped
    with two 16-core Intel Xeon E5-2698 v3 CPUs, which use the Intel Haswell
    microarchitecture.  All nodes have 128 GB of RAM and are connected via a
    Cray Aries interconnect.
    \item NERSC's Cori Phase II supercomputer, a Cray XC40.
    Each node is a self-hosted 68-core Intel Xeon Phi 7250 accelerator, which
    uses the Intel Knights Landing microarchitecture.  All nodes are equipped
    with 96 GB of DRAM and 16 GB of MCDRAM and are connected via a Cray Aries
    interconnect.
    \item NERSC's Edison supercomputer, a Cray XC30.
    Each node is equipped with two 12-core Intel Xeon E5-2695 v2 CPUs,
    which use the Intel Ivy Bridge microarchitecture.  All nodes have 64 GB of
    RAM and are connected via a Cray Aries interconnect.
  \end{itemize}
  \item \textbf{Output} Average and total execution time.
  \item \textbf{Experiment Workflow} Download software, compile from source, run
  the applications, examine the outputs.
  \item \textbf{Publicly available?} Yes.
\end{itemize}

\subsubsection{How software can be obtained (if available)}
\begin{itemize}
  \item \bcl{} can be downloaded from \{omitted for double blind\}.  All
  benchmarks can be found in the examples directory on branch
  \texttt{\{omitted for double blind\}}.
  \item The NERSC Meraculous benchmark can be downloaded from the NERSC website at
  \url{http://www.nersc.gov/research-and-development/apex/apex-benchmarks/meraculous/}.
  \item PapyrusKV with the Meraculous benchmark can be obtained by cloning the Git repository
  at \url{https://code.ornl.gov/eck/papyrus} and checking out commit
  \texttt{11d3e256}.
  \item Chapel can be obtained from \url{https://chapel-lang.org/},
  and the Chapel ISx benchmark can be found in Git repository at
  \url{https://github.com/chapel-lang/chapel} in the directory
  \texttt{test/release/examples/benchmarks/isx}.

  \item The original ISx benchmark reference implementation can be found at
  \url{https://github.com/ParRes/ISx}.
\end{itemize}

\subsubsection{Hardware dependencies}
Reproducing our scaling experiments requires access to a cluster.

\subsubsection{Software dependencies}
To run our \bcl{} benchmarks, a C++-14 compliant compiler and an MPI, SHMEM, or
GASNet implementation.  PapyrusKV requires an MPI implementation with \texttt{MPI\_THREAD\_MULTIPLE}
support.

\subsubsection{Datasets}
Our Meraculous benchmarks use the NERSC Meraculous datasets available at
\url{http://www.nersc.gov/research-and-development/apex/apex-benchmarks/meraculous/}.

\subsection{Installation}
\begin{itemize}
  \item \bcl{} can be installed by ensuring that an MPI, SHMEM, or GASNet backend
  is available, cloning the \bcl{} Git repository at
  \texttt{\{omitted for double blind\}}, checking out branch \texttt{\{omitted for
  double blind\}}, and adding the new directory to the \texttt{CPLUS\_INCLUDE\_PATH}
  environment variable.
  \item Instructions for installing UPC are available at \url{http://upc.lbl.gov/}.
  \item Instructions for installing Chapel are available at \url{https://chapel-lang.org/}.
\end{itemize}

\subsection{Experiment Workflow}
Each \bcl{} benchmark is available in the \texttt{examples/isx-sort} folder of the \bcl{}
Git repository.  Each benchmark can be compiled with the makefile included in its
directory.

\subsubsection{ISx Benchmark}
The \bcl{} ISx benchmark is executed with one rank per core.  On Cori Phase I,
it can be invoked with the command
\texttt{srun -N \$SLURM\_JOB\_NUM\_NODES -n \$((SLURM\_JOB\_NUM\_NODES*32)) ./sort}
to reproduce the results in Figure \ref{fig:isx-sort}.  Instructions for running
the original ISx reference implementation are available at
\url{https://github.com/ParRes/ISx}, and instructions for running Chapel programs
on NERSC are available at
\url{http://www.nersc.gov/users/computational-systems/edison/programming/chapel/}.
The original ISx reference benchmark is invoked with one rank per core,
and the Chapel benchmark is invoked with one locale per node and the
appropriate number of tasks per core on the particular system as outlined in the
NERSC documentation.
\subsubsection{Hypercube Quicksort}
The \bcl{} benchmark is available in the \texttt{examples/hybrid-sort} folder of the
\bcl{} Git repository.  It is executed with one rank per CPU and a thread
for each CPU core.
\subsubsection{Meraculous}
The \bcl{} benchmark is available in the \texttt{example/kmer\_hash} folder of the
\bcl{} Git repository.  It is executed with one rank per core.  Instructions
for executing the original Meraculous UPC implementation can be found at
\url{http://www.nersc.gov/research-and-development/apex/apex-benchmarks/meraculous/}.

